Generalized Shortest Path Kernel on Graphs

We consider the problem of classifying graphs using graph kernels. We define a new graph kernel, called the generalized shortest path kernel, based on the number and length of shortest paths between nodes. For our example classification problem, we consider the task of classifying random graphs from two well-known families, by the number of clusters they contain. We verify empirically that the generalized shortest path kernel outperforms the original shortest path kernel on a number of datasets. We give a theoretical analysis for explaining our experimental results. In particular, we estimate distributions of the expected feature vectors for the shortest path kernel and the generalized shortest path kernel, and we show some evidence explaining why our graph kernel outperforms the shortest path kernel for our graph classification problem.

==> tex/abstract.tex <==
\begin{abstract}
ABSTRACT HERE
\end{abstract}

\begin{comment}
Checklist: 
- new problem
- new approach
- new setting (anonymized)
- extensions 
- results: 
. timing
. 

\end{comment}

==> tex/analysis.tex <==
\section{Analysis}
\label{sec:Analysis}

In this section
we give some approximated analysis of random feature vectors
in order to give theoretical support for our experimental observations.
%OW: observation or observations?
We first show that one-cluster and two-cluster graphs
have quite similar SPI feature vectors (as their expectations).
Then we next show some evidence
that there is a non-negligible difference in their GSPI feature vectors.
Throughout this section,
we consider feature vectors
defined by considering only paths from any fixed source node $s$.
Thus,
for example,
$\numfst{d}$ is the number of nodes at distance $d$ from $s$
in a one-cluster graph,
and $\numsnd{d,x}$ is the number of nodes
that have $x$ shortest paths of length $d$ to $s$ in a two-cluster graph.



Here we introduce a way to state an approximation.
For any functions $a$ and $b$ depending on $n$,
we write
$a\myapprox b$ by which we mean
%
\[
b\left(1-{c\over n}\right)
<a<b\left(1+{c\over n}\right)
\]
%
holds for some constant $c>0$ and sufficiently large $n$.
We say that
$a$ and $b$ are relatively $\myrelclose$-close.
Note that
this closeness notion
is closed under constant number of additions/subtractions and multiplications.
For example,
if $a\myapprox b$ holds,
then we also have $a^k\myapprox b^k$ for any $k\ge1$
that can be regarded as a constant w.r.t.\ $n$.
In the following
we will often use this approximation.
In the following analysis it is important to recall the difference between a walk and a path. A walk is simply a sequence of neighboring nodes, while a path also has the requirement that no node in the path may appear more than once. 

\subsection{Approximate Comparison of SPI Feature Vectors}

Here we consider relatively small\footnote{This smallness assumption is just for simplifying our analysis, and we believe that the situation is more or less the same for any $d$.}
distances $d$
so that $d$ can be considered as a small constant w.r.t.\ $n$.
We show that
$\numEfst{d}$ and $\numEsnd{d}$ are similar in the following sense.

\begin{theorem}
For any constant $d$,
we have
$\numEfst{d}\myapprox\numEsnd{d}$.
%
%\begin{equation}
%\label{eq:theosp}
%\numEfst{d}=\numEsnd{d}\left(1\pm\mathcal{O}\left({1\over n}\right)\right).
%\end{equation}
\end{theorem}

\noindent
{\bf Remark.}~
For deriving this relation
we assume a certain independence
on the existence of two walks in $G$;
see the argument below for the detail.
\bigskip

First consider a one-cluster graph $G=(V,E)$ and analyze $\numEfst{d}$. 
For this analysis,
consider any target node $t$ ($\ne s$) of $G$,
and estimate first the probability $\Ffst_d$
that there exists at least one walk of length $d$ from $s$ to $t$.
Let $A_{u,v}$ be the event that an edge $\{u,v\}$ exists in $G$,
and let $W_d$ denote
the set of
all tuples $(v_1,\ldots,v_{d-1})$ of nodes in $V\setminus\{s\}$
such that $v_i\ne v_{i+1}$ for all $i$, $1\le i\le d-1$,
and $\{v_i,v_{i+1}\}\ne\{v_j,v_{j+1} \}$ for all $i$ and $j$,
$1\le i<j\le d-1$.
(It may be possible that
the same node appears more than once,
but no loop edge appears in the walk, neither does the same edge appear several times in the walk.)
For each tuple $(v_1,\ldots,v_{d-1})$ of $W_d$,
the event $A_{s,v_1}\land A_{v_1,v_2}\land\ldots\land A_{v_{d-1},t}$
is called
the event that
the walk specified by $(s,v_1,\ldots,v_{d-1},t)$ exists in $G$
(or, more simply,
{\em
the existence of one specific walk}).
Then the probability $\Ffst_d$ is expressed by
%
\begin{equation}
\label{eq:Ffst}
\Ffst_d
=\myP\left[\,
\bigvee_{(v_1,\ldots,v_{d-1})\in W_d}
A_{s,v_1}\land A_{v_1,v_2}\land\ldots\land A_{v_{d-1},t}\,\right]
\end{equation}
%
Clearly,
the probability of the existence of one specific walk is $p_1^d$,
and the above probability can be calculated
by using the inclusion-exclusion principle.
Here we follow the analysis of Fronczak et al.~\cite{fronczak2004average}
and assume that
every specific walk exists independently.
Then it is easy to see that
the first term of the inclusion-exclusion principle
is relatively $\myrelclose$-close to $n^{d-1}p_1^{d}$,
and hence, we have
%
\[
\Ffst_d
=
\sum_{(v_1,\ldots,v_{d-1})\in W_d} p_1^d
\myapprox
n^{d-1}p_1^d
\]
%
because $|W_d|$ is relatively $\myrelclose$-close to $n^{d-1}$.
Let $\ffst_d$ be the probability that
$t$ has a shortest path of length $d$ to $s$.
Then due to the disjointness of the two events
(i) $t$ has a shortest path of length $d$ to $s$, 
and (ii) $t$ has a walk of length $d-1$ to $s$,
we have $\ffst_d=\Ffst_d-\Ffst_{d-1}$ for $d\ge2$,
where a similar analysis holds for $\Ffst_{d-1}$.
(For $d=1$,
we have $\ffst_1=\Ffst_1=p_1$.)
Then since $\numEfst{d}=(n-1)\ffst_d$,
we have
%
\[
\numEfst{d}
\myapprox
n^dp_1^d-n^{d-1}p_1^{d-1}.
\]

The argument is similar for a two-cluster graph.
Let us assume first that $s$ is in $V^+$.
Here we need to consider
the case that the target node $t$ is also in $V^+$ and
the case that it is in $V^-$.
Let $\Fsndp_d$ and $\Fsndm_d$  be %Used to just be \Fsndp and \Fsndm. Changed this and equation below to include subscripts
the probabilities that
$t$ has at least one walk of length $d$ to $s$ in the two cases.
Then with a similar analysis,
we have
%
\[
\Fsndp_d
\myapprox
\sum_{{\rm even}~k=0}^{d}\left(n\over2\right)^{d-1}
{d\choose k}p_2^{d-k}q_2^k,
{\rm~~and~~}
\Fsndm_d
\myapprox
\sum_{{\rm odd}~k=1}^{d}\left(n\over2\right)^{d-1}
{d\choose k}p_2^{d-k}q_2^k,
\]
%
and
%
\[
\numEsnd{d}
\myapprox
{n\over2}\bigl(\,\Fsndp_d+\Fsndm_d-(\Fsndp_{d-1}+\Fsndm_{d-1})\,\bigr)
\]

Here we note that
%
\[
\begin{array}{l}
\displaystyle
\sum_{{\rm even}~k=0}^{d}\left(n\over2\right)^{d-1}
{d\choose k}p_2^{d-k}q_2^k
+\sum_{{\rm odd}~k=1}^{d}\left(n\over2\right)^{d-1}
{d\choose k}p_2^{d-k}q_2^k\\
\hspace*{10mm}
\displaystyle
=
\sum_{k=0}^{d}\left(n\over2\right)^{d-1}{d\choose k}p_2^{d-k}q_2^k
=
\left(n\over2\right)^{d-1}(p_2+q_2)^d.
\end{array}
\]
%
and that
$p_2+q_2$ $\myapprox$ $2p_1$ from our choice of $q_2$
(see (\ref{eq:pandq})).
Thus,
$\numEsnd{d}$ is again $\myrelclose$-close to $n^{d}p_1^d - n^{d-1} p_1^{d-1}$, %THIS HAS TO BE VERIFIED.. Used to be n^{d-1}p_1^d ONLY... now I have added a lot more since I believe it's correct.
which proves the theorem.

\subsection{Heuristic Comparison of GSPI Feature Vectors}

We compare the expected GSPI feature vectors $\vecvgspEfst$ and $\vecvgspEsnd$,
and show evidence
that they have some non-negligible difference.
In this section
we focus on the distance $d=2$ part of the GSPI feature vectors,
let $\vecvtwoEz$ denote
the subvector $[\numtwoEz{x}]_{x\ge1}$ of $\vecvgspEz$.
Since it is not so easy to analyze
the distribution of the values $\numtwoEz{1},\numtwoEz{2},\ldots$,
we here introduce some ``heuristic'' analysis.

Again we begin with a one-cluster graph $G$,
and let $V_2$ denote the set of nodes of $G$
with distance 2 from the source node $s$.
Consider any $t$,
and for any $x\ge1$,
we estimate the probability that
it has $x$ number of shortest paths of length 2 to $s$.
Recall that
$G$ has $(n-1)\ffst_1 \myapprox np_1$ nodes %{\bf WAS PRVIOUSLY $(n-1)\Ffst_1$  }
with distance 1 from $s$ on average.
Here we assume that
$G$ indeed has $np_1$ nodes with distance 1 from $s$
and that
an edge between each of these distance 1 nodes and $t$ exists
with probability $p_1$ independently at random.
In other words,
$x$ follows the binomial distribution,
or more precisely,
$x$ is the random variable $\myBin(np_1,p_1)$,
where by $\myBin(N,p)$
we mean a random number of heads that we have
when flipping a coin that gives heads with probability $p$
independently $N$ times.
Then for each $x\ge1$,
$\numtwoEfst{x}$ is estimated by
%
\[
\numtwoEEfst{x}
=
\sum_{t\in V_2}\myP\bigl[\,\myBin(np_1,p_1)=x\,\bigr]
=
\numEfst{2}
\cdot
\myP\bigl[\,\myBin(np_1,p_1)=x\,\bigr],
\]
%
by assuming again
that $|V_2|$ is its expected value $\numEfst{2}$.
Clearly
the distribution of values of vector $[\numtwoEEfst{x}]_{x\ge1}$
is proportional to $\myBin(np_1,p_1)$,
and it has one peak at $\xpeakfst=np_1^2$.

Consider now a two-cluster graph $G$.
For $d\in\{1,2\}$,
let $V_d^+$ and $V_d^-$ denote respectively
the set of nodes in $V^+$ and $V^-$ with distance $d$ from $s$.
Let $V_2=V_2^+\cup V_2^-$.
Again we assume that
$V_1^+$ and $V_1^-$ have respectively $np_2/2$ and $nq_2/2$ nodes
and that
the numbers of edges
from $V_1^+$ and $V_1^-$ to a node in $V_2$ follow binomial distributions.
We once again assume that $s \in V^+$.
Note that we need to consider two cases here.
First consider the case that the target node $t$ is in $V_2^+$.
In this case,
we have
%
\begin{eqnarray*}
\ptwosndp{x}
&:=&
\myP\bigl[\,\mbox{$t$ has $x$ shortest paths}\,\bigr]\\
&=&
\myP\left[\,\myBin\left({n\over2}p_2,p_2\right)
+\myBin\left({n\over2}q_2,q_2\right)=x\,\right]\\
&\approx&
\myP\left[\,\myN\left({n\over2}(p_2)^2,\sigma_1^2\right)
+\myN\left({n\over2}(q_2)^2,\sigma_2^2\right)=x\,\right]\\
&=&
\myP\left[\,\myN
\left({n((p_2)^2+(q_2)^2)\over2},\sigma_1^2+\sigma_2^2\right)=x\right],
\end{eqnarray*}
%
where we use the
normal distribution $\myN(\mu,\sigma^2)$
to approximate each binomial distribution
so that we can express their sum by a normal distribution
(here we omit specifying $\sigma_1$ and $\sigma_2$).
The case where $t\in V^-_2$ can be analyzed similarly,
and we obtain that
%
\[
\ptwosndm{x}
:=
\myP\bigl[\,\mbox{$t$ has $x$ shortest paths}\,\bigr]
=
\myP\left[\,\myN
\left(np_2q_2,\sigma_3^2 + \sigma_4^2 \right)=x\right].
\]
%
Then again we may estimate $\numtwoEsnd{x}$
by $\numtwoEEsnd{x}$ $:=$ $\myE[V_2^+]\ptwosndp{x}+\myE[V_2^-]\ptwosndm{x}$.

We have now arrived at the key point in our analysis. Note that 
$\numtwoEEsnd{x}$ now follows the mixture of two distributions,
namely,
$\myN(n((p_2)^2+(q_2)^2)/2,\sigma_1^2+\sigma_2^2)$
and $\myN(np_2q_2,\sigma_3^2 + \sigma_4^2)$, with weights $\myE[V_2^+]/(\myE[V_2^+] + \myE[V_2^-] )$ and  $\myE[V_2^-] /(\myE[V_2^+] + \myE[V_2^-] )$.
Now we estimate
the distance between the two peaks $\xpeaksndp$ and $\xpeaksndm$
of these two distributions.
Then we have
%
\begin{eqnarray*}
2(\xpeaksndp-\xpeaksndm)
&=&
n(p_2^2+q_2^2-2p_2q_2)
=
n(p_2-q_2)^2\\
&\myapprox&
n(p_2-(2p_1-p_2))^2
=
4n\alpha_0^2p_1^2.
\end{eqnarray*}
%
From this we have
%
\[
\xpeaksndp
\myapprox
\xpeaksndm\left(1+{2n\alpha_0^2p_1^2\over\xpeaksndm}\right)
>(1+2\alpha_0^2)\xpeaksndm.
\]
%
Therefore these peaks have non-negligible relative difference,
which indicates that
two vectors $\vecvtwoEfst$ and $\vecvtwoEsnd$
have different distributions of their component values. In particular $\vecvtwoEfst$ will only have one peak, while $\vecvtwoEsnd$ will have a double peak shape (for large enough $\alpha_0)$.
Though this is a heuristic analysis,
we can show some examples that
our heuristic analysis is not so different
from experimental results. In Fig. \ref{fig:exp_approx} we have plotted both our approximated vector $\vecvtwoEsnd$ (actually we have plotted the normal distribution that gives this vector) and the corresponding experimental vector obtained by generating graphs according to our random model. In this figure the double peak phenomena can clearly be observed, which provides empirical evidence that our analysis is sound. 
The experimental vector is the average vector for each fixed source node in the graph and averaged over 500 randomly generated graphs, where the graphs were generated with the parameters $n=400, p_2=0.18, q_2=0.0204$.



\begin{figure}[tb]
\centering
    \includegraphics[width=1.0\columnwidth, keepaspectratio=true]{img/exp_approx1.png}
\caption{%
Average experimental and approximate distributions of number of nodes with $x$ number of shortest paths of length 2 to a fixed node. The experimental distribution has been averaged for each node in the graph and also averaged over 500 randomly generated graphs. The graphs used had parameters $n=400$, $p_2=0.18$ and $q_2=0.0204$. (For computing the graph of the 
approximate distribution,
we used a more precise approximation for,
e.g., $\myE[V_2^+]$ because our $n$ is not
large enough.)
}
\label{fig:exp_approx}
\end{figure}




